Towards Math-Aware Automated Classification and Similarity Search of Scientific Publications: Methods of Mathematical Content Representations

In this paper, we investigate mathematical content representations suitable for the automated classification of and the similarity search in STEM documents using standard machine learning algorithms: the Latent Dirichlet Allocation (LDA) and the Latent Semantic Indexing (LSI). The methods are evaluated on a subset of arXiv.org papers with the Mathematics Subject Classification (MSC) as a reference classification and using the standard precision/recall/F1-measure metrics. The results give insight into how different math representations may influence the performance of the classification and similarity search tasks in STEM repositories. Non-surprisingly, machine learning methods are able to grab distributional semantics from textual tokens. A proper selection of weighted tokens representing math may improve the quality of the results slightly. A structured math representation that imitates successful text-processing techniques with math is shown to yield better results than flat TeX tokens.

==> Makefile <==
# $Id: Makefile 2281 2017-03-22 13:10:09Z ruzicka $

RUN_COUNT=3
NAME=cicm-2017

DOCUMENT_DEPENDENCIES=${NAME}.tex table-*.tex ${NAME}.bib *.cls *.bst picture-* Makefile
DOCUMENT_OUTPUTS=${NAME}.pdf
DOCUMENT_METADATA=${NAME}.{aux,bbl,blg,idx,ilg,ind,lof,log,nav,out,snm,vrb,toc}

SHELL=/bin/bash
PDF_PRODUCER=${ENVIRONMENT} pdflatex
ifeq (${RUN_COUNT}, 1)
  PDF_EXTRA_ARGUMENTS=-draftmode -interaction batchmode
else
  PDF_EXTRA_ARGUMENTS=
endif

PDF_PRODUCER_ARGUMENTS=
BIBTEX=biber
BIBTEX_ARGUMENTS=
INDEX_PRODUCER=${ENVIRONMENT} makeindex
INDEX_PRODUCER_ARGUMENTS=


.PHONY: all pdf clean

default: pdf
all: pdf
pdf: ${NAME}.pdf

clean:
	@echo -e "\n### CLEAN... ###"
	-rm ${DOCUMENT_OUTPUTS} ${DOCUMENT_METADATA}
	@echo -e "### CLEAN DONE. ###"

${NAME}.pdf: ${DOCUMENT_DEPENDENCIES}
	@echo -e "\n### PDF... ###"
	@echo -e "\n### PDF METADATA CLEAN... ###"
	-rm ${DOCUMENT_METADATA}
	@echo -e "### PDF METADATA CLEAN DONE. ###"
	@echo -e "\n### PDF COMPILATION... ###"
	${PDF_PRODUCER} ${PDF_PRODUCER_ARGUMENTS} ${PDF_EXTRA_ARGUMENTS} ${NAME}.tex
ifneq (${RUN_COUNT}, 1)
	${BIBTEX} ${BIBTEX_ARGUMENTS} ${NAME}
#	${INDEX_PRODUCER} ${INDEX_PRODUCER_ARGUMENTS} ${NAME}.idx
	for i in `seq $$[${RUN_COUNT}-1]`; do \
		echo; \
		${PDF_PRODUCER} ${PDF_PRODUCER_ARGUMENTS} ${NAME}.tex; \
	#	if [ $${i} -ne $$[${RUN_COUNT}-1] ]; then \
	#		${INDEX_PRODUCER} ${INDEX_PRODUCER_ARGUMENTS} ${NAME}.idx; \
	#	fi; \
	done
endif
	@echo -e "### PDF COMPILATION DONE. ###"
	@echo -e "\n### PDF DONE. ###"

query-stats-agregated.tex: query-stats-generator.pl query-stats.csv
	./query-stats-generator.pl < query-stats.csv > query-stats-agregated.tex

query-stats.csv:
	for i in ../../../../software/NTCIR-results-processing/NTCIR-11/outputs/2014-06-16T18-16-20*.response.xml; do \
		echo -n "$${i}" | \
			sed 's/^.*....-..-..T..-..-.._MIRMU_\([^_]\+\)_\([^\.]\+\)\.\([[:digit:]]\+\)\.response.xml/\1,\2,\3/g'; \
		echo -ne ','; \
		xmlstarlet sel -t -v '/results/time' -n "$${i}"; \
	done > query-stats.csv

results-stats-agregated.csv: results-stats-generator.pl results-stats.csv
	./results-stats-generator.pl < results-stats.csv > results-stats-agregated.csv

results-stats.csv:
	for i in ../../../../software/NTCIR-results-processing/NTCIR-11/outputs/2014-06-16T18-16-20*.response.xml; do \
		echo -n "$${i}" | \
			sed 's/^.*....-..-..T..-..-.._MIRMU_\([^_]\+\)_\([^\.]\+\)\.\([[:digit:]]\+\)\.response.xml/\1,\2,\3/g'; \
		echo -ne ','; \
		xmlstarlet sel -t -v 'count(/results/result)' -n "$${i}"; \
	done > results-stats.csv

